Physics-Guided Problem Decomposition for Scaling Deep Learning of High-dimensional Eigen-Solvers: The Case of Schr\"{o}dinger's Equation

Given their ability to effectively learn non-linear mappings and perform fast inference, deep neural networks (NNs) have been proposed as a viable alternative to traditional simulation-driven approaches for solving high-dimensional eigenvalue equations (HDEs), which are the foundation for many scientific applications. Unfortunately, for the learned models in these scientific applications to achieve generalization, a large, diverse, and preferably annotated dataset is typically needed and is computationally expensive to obtain. Furthermore, the learned models tend to be memory- and compute-intensive primarily due to the size of the output layer. While generalization, especially extrapolation, with scarce data has been attempted by imposing physical constraints in the form of physics loss, the problem of model scalability has remained. In this paper, we alleviate the compute bottleneck in the output layer by using physics knowledge to decompose the complex regression task of predicting the high-dimensional eigenvectors into multiple simpler sub-tasks, each of which are learned by a simple "expert" network. We call the resulting architecture of specialized experts Physics-Guided Mixture-of-Experts (PG-MoE). We demonstrate the efficacy of such physics-guided problem decomposition for the case of the Schr\"{o}dinger's Equation in Quantum Mechanics. Our proposed PG-MoE model predicts the ground-state solution, i.e., the eigenvector that corresponds to the smallest possible eigenvalue. The model is 150x smaller than the network trained to learn the complex task while being competitive in generalization. To improve the generalization of the PG-MoE, we also employ a physics-guided loss function based on variational energy, which by quantum mechanics principles is minimized iff the output is the ground-state solution.

==> misc.tex <==
% Minor comments
- PG-loss or PG loss? Whichever version we like, we should be consistent with that throughout the paper.
- Is it necessary to always write CS in the table's caption? I have done it for all but Idk that's necessary.


% From Prof
2/8
- Why the kind of architectural decomposition we are doing is better than existing PINN work?
- How does our problem compare to the other problems that people have studied? (Does scaling with N show up in existing works? In any case, we need to compare with other PINNs works)
- How does the scalability change for 2-d system? We have considered a 1-d Ising model.
- Future work: 
    - alternate neural architectures for experts? See if you can find anything relevant from the PINN work.
    - data curation; memory required to store Hamiltonian for PG loss
    - local loss/local invariance for a more stable arch? will also make the training of experts independently.


% Reference:
All results can be found in the following Google sheet.
https://docs.google.com/spreadsheets/d/1A0s87tBTe1eHdY0nlU87EtFR7rYcehonG6EO5iQJqSE/edit#gid=1724368561





==> table5.tex <==
\begin{table*}[]
\begin{tabular}{l|l|c|cr|cr}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Architecture}}} & \multirow{2}{*}{\textbf{\#params}} & \multicolumn{2}{c|}{\textbf{CS (w/o $L_{PG}$)}} & \multicolumn{2}{c}{\textbf{CS (with $L_{PG}$)}} \\ \cline{4-7} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{$B_x \!< 1$} & \multicolumn{1}{c|}{$B_x \!> 1$} & \multicolumn{1}{c|}{$B_x \!< 1$} & \multicolumn{1}{c}{$B_x \!> 1$} \\ \hline
\textbf{Baseline} & d\_2\_n\_2000 & \multicolumn{1}{r|}{6093024} & \multicolumn{1}{r}{$0.996\pm0.0008$} & $0.874\pm0.0028$ & \multicolumn{1}{r}{$1.000\pm0.000$} & $0.981\pm0.0003$ \\
\textbf{PG-MoE} & d\_2\_n\_200 & \multicolumn{1}{r|}{39903} & \multicolumn{1}{r}{$0.996\pm0.0008$} & ${0.882\pm0.0083}$ & \multicolumn{1}{r}{$1.000\pm0.000$} & ${0.977\pm0.0044}$ \\ \hline
\end{tabular}
\caption{Comparison of cosine similarity (CS) of the Baseline and PG-MoE networks on the $D_T$ ($B_x \!< 1$) and $D_{UT}$ ($B_x \!> 1$) test sets. $d$ and $n$ correspond to the number of hidden layers and the number of neurons in each layer of the NN.}
\label{tbl:pg-moe}
\end{table*}
